Preface: A Data-driven Volumetric Prior for Few-shot Ultra High-resolution Face Synthesis

NeRFs have enabled highly realistic synthesis of human faces including complex appearance and reflectance effects of hair and skin. These methods typically require a large number of multi-view input images, making the process hardware intensive and cumbersome, limiting applicability to unconstrained settings. We propose a novel volumetric human face prior that enables the synthesis of ultra high-resolution novel views of subjects that are not part of the prior's training distribution. This prior model consists of an identity-conditioned NeRF, trained on a dataset of low-resolution multi-view images of diverse humans with known camera calibration. A simple sparse landmark-based 3D alignment of the training dataset allows our model to learn a smooth latent space of geometry and appearance despite a limited number of training identities. A high-quality volumetric representation of a novel subject can be obtained by model fitting to 2 or 3 camera views of arbitrary resolution. Importantly, our method requires as few as two views of casually captured images as input at inference time.

==> figures/01_method_teaser.tex <==
\begin{figure*}[t]
    \centering
  \includegraphics[width=\textwidth]
                  {figures/01_method_teaser}
    \caption{Our key contribution is an implicit prior face model (left), learned from a novel multiview dataset of faces captured in a controlled setting. The prior model is resolution independent and can be fine-tuned to synthesise novel views in ultra-high resolution given as few as 2 images from a target identity captured in-the-wild (right).
    \label{fig:method_teaser}}
\end{figure*}

==> figures/comparison/comparison_holobooth_full.tex <==
\begin{figure*}[ht]

\begin{center}
\small
\setlength{\tabcolsep}{2pt}

\newcommand{\height}{3cm}
\begin{tabular}{cccccc}
& \textbf{Subject A}\\
\rotatebox{90}{RegNeRF}
  & \includegraphics[height=\height]
 {figures/comparison/holobooth/regnerf_in2_0_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/regnerf_in3_0_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/regnerf_in5_0_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/regnerf_in7_0_pred} 
    \\    
\rotatebox{90}{FreeNeRF}
  & \includegraphics[height=\height]
 {figures/comparison/holobooth/freenerf_in2_0_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/freenerf_in3_0_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/freenerf_in5_0_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/freenerf_in7_0_pred} 
    \\    
\rotatebox{90}{\textbf{Ours}} & \includegraphics[height=\height]{figures/comparison/holobooth/ours_in2_0_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/ours_in3_0_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/ours_in5_0_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/ours_in7_0_pred} 
    \\
& \textbf{Subject B}\\
 \rotatebox{90}{RegNeRF}& \includegraphics[height=\height]
{figures/comparison/holobooth/regnerf_in2_2_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/regnerf_in3_2_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/regnerf_in5_2_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/regnerf_in7_2_pred} 
   \\
\rotatebox{90}{FreeNeRF}
  & \includegraphics[height=\height]
 {figures/comparison/holobooth/freenerf_in2_2_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/freenerf_in3_2_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/freenerf_in5_2_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/freenerf_in7_2_pred} 
    \\    
\rotatebox{90}{\textbf{Ours}} & \includegraphics[height=\height]{figures/comparison/holobooth/ours_in2_2_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/ours_in3_2_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/ours_in5_2_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/ours_in7_2_pred} 
    \\    
& \textbf{Subject C}\\
\rotatebox{90}{RegNeRF}
 &\includegraphics[height=\height]
{figures/comparison/holobooth/regnerf_in2_1_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/regnerf_in3_1_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/regnerf_in5_1_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/regnerf_in7_1_pred} 
    \\    
\rotatebox{90}{FreeNeRF}
  & \includegraphics[height=\height]
 {figures/comparison/holobooth/freenerf_in2_1_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/freenerf_in3_1_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/freenerf_in5_1_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/freenerf_in7_1_pred} 
    \\    
\rotatebox{90}{\textbf{Ours}} & \includegraphics[height=\height]{figures/comparison/holobooth/ours_in2_1_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/ours_in3_1_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/ours_in5_1_pred} 
    & \includegraphics[height=\height]{figures/comparison/holobooth/ours_in7_1_pred} 
    \\
    
& 2 Views & 3 Views & 5 Views & 7 Views 
\end{tabular}
\end{center}

\caption{\label{fig:comparison_1k} Visual comparison on our dataset. We compare with RegNeRF~\cite{regnerf} and FreeNeRF~\cite{Yang2023FreeNeRF} for different number of views, ranging from 2 to 7. Our method consistency produces more pleasing results. Please see Tbl.~\ref{tbl:regnerf} for metrics. Subject A, B, and C in the table correspond to the first, second, and third example in this grid.}

\end{figure*}

==> tables/ablation_expression.tex <==
\begin{table}[!h]
\small 
\begin{center}
\begin{tabular}{c | ccc}
\hline
\multicolumn{3}{c}{\textbf{Expression}}\\ 
    \multicolumn{1}{c}{\textbf{PSNR} $\uparrow$} &
    \multicolumn{1}{c}{\textbf{SSIM} $\uparrow$} & 
    \multicolumn{1}{c}{\textbf{LPIPS} $\downarrow$}\\
\hline
\end{tabular}
\end{center}
\caption{TODO}
\label{tab:ablation_expression}
\end{table}

==> tables/ablation_lighting.tex <==
\begin{table}[!h]
\small 
\begin{center}
\begin{tabular}{l ccc}
\hline
\textbf{Lighting} &
    \multicolumn{1}{c}{\textbf{PSNR} $\uparrow$} &
    \multicolumn{1}{c}{\textbf{SSIM} $\uparrow$} & 
    \multicolumn{1}{c}{\textbf{LPIPS} $\downarrow$}\\
    \hline
    A) Fully Lit & 25.87 & 0.7688 & 0.1978 \\
    B) Medium Shadows & 28.53 & 0.8500 & 0.2002 \\
    C) Strong Shadows & 28.75 & 0.8480 & 0.1952 \\
\end{tabular}
\end{center}
\caption{Performance under strong lighting conditions. \Rfour{} Our model robustly synthesises high-quality novel views. We provide visual results for novel views in Fig.~\ref{fig:ablation_lighting}.\MB{The metrics for 'fully lit' are worse because the fully lit image shows more details and reconstructing these is a harder task.}}
\label{tab:ablation_lighting}
\end{table}
